VideoCogQA: A Controllable Benchmark for Evaluating Cognitive Abilities in Video-Language Models

Recent advancements in Large Video-Language Models (LVLMs) have led to promising results in multimodal video understanding. However, it remains unclear whether these models possess the cognitive capabilities required for high-level tasks, particularly those involving symbolic and abstract perception. Existing benchmarks typically rely on real-world, annotated videos, which lack control over video content and inherent difficulty, limiting their diagnostic power. To bridge this gap, we propose VideoCogQA, a scalable and fully controllable benchmark inspired by game-world environments, designed to evaluate the cognitive abilities of LVLMs. By generating synthetic videos via a programmatic engine, VideoCogQA allows fine-grained control over visual elements, temporal dynamics, and task difficulty. This approach enables a focused evaluation of video cognitive abilities, independent of prior knowledge from visual scene semantics. The dataset includes 800 videos and 3,280 question-answer pairs, featuring tasks related to abstract concepts, symbolic elements, and multimodal integration, with varying levels of difficulty. Experimental results show that even state-of-the-art (SOTA) models, such as GPT-4o, achieve an average performance of 48.8% on tasks involving abstract concepts. Additionally, performance drops by 15% as task complexity increases, highlighting the challenges LVLMs face in maintaining consistent performance. Through this work, we hope to show the limitations of current LVLMs and offer insights into how they can more effectively emulate human cognitive processes in the future.

==> latex/case10.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{latex/pdf/scenes2.pdf}
    \caption{In the \textit{Sky Battle} scene, symbolic icons represent players, bullets, and enemies, while the action "destroy" is abstractly portrayed. The difficulty level is adjusted by varying the number and speed of enemy symbols. Questions such as “How many enemies were destroyed by player?” are used to test the model’s perception of game scenes.}
    \label{SKBCASES}
\end{figure*}

% Frames from the "Sky Battle".

==> latex/case10_video.tex <==

\begin{figure*}[ht]
    \centering
    \begin{tabular}{c}
     \hline
        \includegraphics[width=0.4\textwidth]{latex/pdf/scene10.pdf} \\
        % (a) Easy \\
        \\
         \hline
        \begin{minipage}[t]{0.9\textwidth}
            \centering
            \textbf{Question:} How many different notes
were played in total? \\
            (A) 4 \quad (B) 3 \quad (C) 5 \quad (D) 2
        \end{minipage}
        \\
         \hline
    \end{tabular}
    \caption{Example of the 'Note Matcher' scene at the Easy difficulty level with the corresponding QA example.}
    \label{fig:Sound and Vision}
\end{figure*}


==> latex/case11.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{latex/pdf/case_maze.pdf}
    \caption{The case in the Maze Navigation scene.}
    \label{fig:maze_case}
    
\end{figure}

==> latex/case1_video.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.92\linewidth]{sec/pdf/case.pdf}
%     \caption{Data pipeline.}
%     \label{overview of the pipeline}
% \end{figure*}

\begin{figure*}[ht]
    \centering
    \begin{tabular}{c|c|c}
    \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
                Question: In all the scenes, how many times did the red circle appear? \\
                (A) 0 \quad (B)  14 \quad (C) 26 \quad (D) 18
            \end{minipage}
            
        } \\
        \hline
    \end{tabular}
    
    \caption{Case of the 'Chameleon Grid' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:grid_diversity}
\end{figure*}




==> latex/case2_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{ccc}
        \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene2_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene2_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene2_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \\
            \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
                Question: How many objects are performing the 'vertical\_move' action in this scene? \\
                (A) 0 \quad (B)  2 \quad (C) 6 \quad (D) 8
            \end{minipage}
        }\\
            \hline
    \end{tabular}
    \caption{Case of the 'Action Arena' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:Dance of Actions}
\end{figure*}


==> latex/case3_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{ccc}
        \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene3_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene3_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene3_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \\
            \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
                Question: Which object moves faster: the Green circle or the Blue circle? \\
                (A) Green circle \quad (B)  Blue circle \quad (C) Both are equal 
            \end{minipage}
        }\\
            \hline
    \end{tabular}
    \caption{Case of the 'Straight Paths' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:Straight Paths}
\end{figure*}


==> latex/case4_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{c}
        \hline
        \includegraphics[width=0.4\textwidth]{latex/pdf/scene4.pdf} \\
       
        \\
            \hline
        \begin{minipage}[t]{0.9\textwidth}
            \centering
            \textbf{Question:} What object is displayed when the time shows 21:49:21? \\
            (A) Green circle \quad (B) Blue circle \quad (C) Blue Square \quad (D) Red Square
        \end{minipage} \\
            \hline
    \end{tabular}
    \caption{Example of the 'Time Sequence' scene at the Easy difficulty level with the corresponding QA example.}
    \label{fig:Moments in Time}
\end{figure*}


==> latex/case5_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{ccc}
        \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene5_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene5_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene5_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \\
            \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
              For the second occurrence of the object, what is the object in the adjacent cell to the left? \\
                (A) Green circle \quad (B) Red circle \quad (C) Both are equal 
            \end{minipage}
        }
        \\
            \hline
    \end{tabular}
    \caption{Case of the ' Flash Grid' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:Shifting Spaces}
\end{figure*}


==> latex/case6_video.tex <==

\begin{figure*}[ht]
    \centering
    
    \begin{tabular}{c}
        \hline
        \includegraphics[width=0.4\textwidth]{latex/pdf/scene6.pdf} \\

        \\
            \hline
        \begin{minipage}[t]{0.9\textwidth}
            \centering
            \textbf{Question:} Which edge has been traversed the most times? \\
            (A) AB \quad (B) BC \quad (C) CD \quad (D) EF
        \end{minipage}
        \\
        \hline
    \end{tabular}

    \caption{Example of the '3D Navigator' scene at the Easy difficulty level with the corresponding QA example.}
    \label{fig: journey Along Edges}
\end{figure*}


==> latex/case7_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{ccc}
        
        \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene7_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene7_medium.pdf} &
        \includegraphics[width=0.33\textwidth]{latex/pdf/scene7_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \\
         \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
               How many enemies appeared in the video? \\
                (A) 6 \quad (B)  8 \quad (C) 12 \quad (D) 3 
            \end{minipage}
        }
                \\
        \hline
    \end{tabular}
    \caption{Case of the 'Sky Battle' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:Sky Battle}
\end{figure*}

==> latex/case8_video.tex <==

\begin{figure*}[ht]
    \centering
    \begin{tabular}{c}
     \hline
        \includegraphics[width=0.4\textwidth]{latex/pdf/scene9.pdf} \\
      
        \\
         \hline
        \begin{minipage}[t]{0.9\textwidth}
            \centering
            \textbf{Question:} How many moves did each
player make? \\
            (A) 2,1 \quad (B) 4,3 \quad (C) 5,2 \quad (D) 3,2
        \end{minipage}
        \\
         \hline
    \end{tabular}
    \caption{Example of the 'Tic-Tac-Toe Game' scene at the Easy difficulty level with the corresponding QA example.}
    \label{fig:ic-Tac-Toe Game}
\end{figure*}


==> latex/case9_video.tex <==
\begin{figure*}[ht]
    \centering
    \begin{tabular}{c|c|c}
        \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene8_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene8_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene8_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
                \textbf{Question:} How many steps did the player take to solve the maze? \\
                (A) 8 \quad (B) 9 \quad (C) 4 
            \end{minipage}
        } \\
        \hline
    \end{tabular}
  \caption{Example of the ' Maze Runner' scene at different difficulty levels, along with the corresponding QA example.}
    \label{fig:MazeNavigation}
\end{figure*}


==> latex/pdf/case1_video.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.92\linewidth]{sec/pdf/case.pdf}
%     \caption{Data pipeline.}
%     \label{overview of the pipeline}
% \end{figure*}

\begin{figure*}[ht]
    \centering
    \begin{tabular}{c|c|c}
    \hline
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_easy.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_medium.pdf} &
        \includegraphics[width=0.3\textwidth]{latex/pdf/scene1_diff.pdf} \\
        (a) Easy & (b) Medium & (c) Hard \\
        \hline
        \multicolumn{3}{c}{
            \begin{minipage}[t]{0.9\textwidth}
                \centering
                Question: In all the scenes, how many times did the red circle appear? \\
                (A) 0 \quad (B)  14 \quad (C) 26 \quad (D) 18
            \end{minipage}
            
        } \\
        \hline
    \end{tabular}
    
    \caption{Case of the 'Chameleon Grid' scene at different difficulty levels with the corresponding QA example.}
    \label{fig:grid_diversity}
\end{figure*}



